Embracing Unknown Step by Step: Towards Reliable Sparse Training in Real World

Sparse training has emerged as a promising method for resource-efficient deep neural networks (DNNs) in real-world applications. However, the reliability of sparse models remains a crucial concern, particularly in detecting unknown out-of-distribution (OOD) data. This study addresses the knowledge gap by investigating the reliability of sparse training from an OOD perspective and reveals that sparse training exacerbates OOD unreliability. The lack of unknown information and the sparse constraints hinder the effective exploration of weight space and accurate differentiation between known and unknown knowledge. To tackle these challenges, we propose a new unknown-aware sparse training method, which incorporates a loss modification, auto-tuning strategy, and a voting scheme to guide weight space exploration and mitigate confusion between known and unknown information without incurring significant additional costs or requiring access to additional OOD data. Theoretical insights demonstrate how our method reduces model confidence when faced with OOD samples. Empirical experiments across multiple datasets, model architectures, and sparsity levels validate the effectiveness of our method, with improvements of up to \textbf{8.4\%} in AUROC while maintaining comparable or higher accuracy and calibration. This research enhances the understanding and readiness of sparse DNNs for deployment in resource-limited applications. Our code is available on: \url{https://github.com/StevenBoys/MOON}.

==> sections/_checklist.tex <==
\section{Checklist}







\begin{itemize}
    \item Have you read the publication ethics guidelines and ensured that your paper conforms to them? \textcolor{blue}{[Yes]}
    \item Did you discuss any potential negative societal impacts (for example, disinformation, privacy, fairness) of your work? \textcolor{gray}{[N/A]}
    \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
        \begin{itemize}
            \item If your work uses existing assets, did you cite the creators and the version?  \textcolor{blue}{[Yes]}
            \item Did you mention the license of the assets? \textcolor{gray}{[N/A]}
            \item Did you include any new assets either in the supplemental material or as a URL? \textcolor{gray}{[N/A]}
            \item Where possible, discuss whether and how consent was obtained from people whose data you're using/curating  \textcolor{gray}{[N/A]}
            \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?  \textcolor{gray}{[N/A]}
        \end{itemize}
    \item If you used crowdsourcing or conducted research with human subjects...
        \begin{itemize}
            \item Did you include the instructions given to participants including the consent form? \textcolor{gray}{[N/A]}
            \item Did you describe any potential participant risks? \textcolor{gray}{[N/A]}
            \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \textcolor{gray}{[N/A]}
        \end{itemize}
    \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \textcolor{blue}{[Yes]}
    \item Did you describe the limitations of your work? \textcolor{blue}{[Yes]}
    \item If you are including theoretical results...
        \begin{itemize}
            \item Did you state the full set of assumptions of all theoretical results? \textcolor{blue}{[Yes]}
            \item Did you include complete proofs of all theoretical results? \textcolor{blue}{[Yes]}
        \end{itemize}
    \item If you ran experiments...
        \begin{itemize}
            \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL, in an anonymized way at the review time)? \textcolor{blue}{[Yes]}
            \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \textcolor{blue}{[Yes]}
            \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \textcolor{blue}{[Yes]}
            \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \textcolor{blue}{[Yes]}
        \end{itemize}
\end{itemize}












